Sound and Complete Proof Rules for Probabilistic Termination

Deciding termination is a fundamental problem in the analysis of probabilistic imperative programs. We consider the qualitative and quantitative probabilistic termination problems for an imperative programming model with discrete probabilistic choice and demonic bounded nondeterminism. The qualitative question asks if the program terminates almost-surely, no matter how nondeterminism is resolved. The quantitative question asks for a bound on the probability of termination. Despite a long and rich literature on the topic, no sound and relatively complete proof systems were known for these problems. In this paper, we provide such sound and relatively complete proof rules for proving qualitative and quantitative termination in the assertion language of arithmetic. Our rules use supermartingales as estimates of the likelihood of a program's evolution and variants as measures of distances to termination. Our key insight is our completeness result, which shows how to construct a suitable supermartingales from an almost-surely terminating program. We also show that proofs of termination in many existing proof systems can be transformed to proofs in our system, pointing to its applicability in practice. As an application of our proof rule, we show an explicit proof of almost-sure termination for the two-dimensional random walker.

==> Makefile <==
SOURCE = main.tex

popl: $(SOURCE) Makefile
	latexmk -pdf main
# 	PAGESBIB=`cat main.pagesbib.ctr`; \ # Don't think it's necessary now
# 		pdftk main.pdf cat 1-$$PAGESBIB output popl.pdf; \
# 		START=`expr $$PAGESBIB + 1`; \
# 		pdftk main.pdf cat $$START-end output supplemental.pdf

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusions}

We have presented the first sound and relatively complete proof rules for qualitative and quantitative termination of probabilistic programs with bounded probabilistic and nondeterministic choice.
Our proof rules combine the familiar ingredients of supermartingales and variant functions in novel ways to reach completeness.
We have demonstrated relative completeness of our rules in the assertion language of arithmetic.
% this is surprising, given the existence of some programs that terminate with transcendental probability values and others that appear to require ordinals to demonstrate termination.
Our rules are able to accommodate existing proof techniques in the literature with minimal effort, thus demonstrating their applicability.

==> mainproofs.tex <==
%Here, I promise to discuss the flaw

\section{Our rules}

\subsection{The issue with Chatterjee's rule}

==> our_rules.tex <==
% I think it makes sense to talk about the quantitative termination case first, and maybe present the AST rule as a special case of the quantitative termination case.

% Also, I can make the probability distributions countable, but the nondeterministic stuff has to still be bounded. But, in our program model, the probabilistic branching is automatically bounded. Adding the assignment of distributions seems to only make things more complicated.

\section{Complete rules for termination}

In this section, we detail sound and complete rules for upper and lower bounds on termination probabilities, and two special rules for determining if a program is $\AST$.


% I separately note: if $(SI, p)$ is a stochastic invariant, then $(SI \cup \{\sigma\}, p)$ is also a stochastic invariant.


We now use the following from \cite[Appendix B]{OurPastPaper} to enable the proof of the completeness of our lower bounds rule.
\begin{definition}
    \label{def:required-simulation-time}
    Let $\cG = (L, V, l_{init}, \allowbreak \bfx_{init}, \ordMapsTo, G, \sfPr, \sfUp)$ be an $\iCFG$ such that $\termProb(\cG) \geq p$.
    For a scheduler $f$, let $(\pi_1, \pi_2, \ldots)$ be an ordering of the terminating runs of $\cG$ induced by $f$ such that $|\pi_1| \leq |\pi_2| \leq \cdots$.
    For some $\epsilon > 0$, let $i_n$ be the smallest number such that
    $$
    p_f(\pi_1) + \cdots + p_f(\pi_{i_n}) \geq p - \epsilon
    $$
    where $p_f$ is the probability measure induced by $f$ over the set of all runs of $\cG$.

    Then, $\pi_n$ is the \emph{required simulation time} of $\cG$ under $f$ to assimilate a termination probability of $p - \epsilon$.
\end{definition}
The required simulation time is simply the length of the longest terminating run that must be accounted for in the termination probability series for it to cross $p - \epsilon$.
\begin{lemma}[\cite{OurPastPaper}]
    \label{lem:required-simulation-time}
    Let $\cG = (L, V, l_{init}, \allowbreak \bfx_{init}, \ordMapsTo, G, \sfPr, \sfUp)$ be an $\iCFG$ such that $\termProb(\cG) \geq p$.
    For any $\epsilon$, the set of all required simulation times across all schedulers is bounded above.
\end{lemma}
\cref{lem:required-simulation-time} is a simple generalization of Lemma B.3 of \citet{OurPastPaper}.
It holds for $\iCFG$s because the branching at nondeterministic locations is bounded.


This complete rule for lower bounds can be used as a rule for $\AST$, by requiring a lower bound of $1$ on the termination probability.
Nevertheless, because of certain properties of $\AST$, we present two proof rules for $\AST$ that exploit these properties.






==> prev_limitations.tex <==
\section{Limitations of Prior Rules}
\label{sec:limitations-chatterjee}

Limitations for the variant rule \cref{proofrule:ast-variant} have been discussed by \citet{McIverMKK18}, along with a few fixes.
The unbiased 1-D random walker suffices as an example of a program for which the rule cannot apply; we leave the details to the reader.

% I can also add a note on the limitations of the $\AST$ rule of Katoen et. al. 2018; I'll leave that for later work.

==> previous_rules.tex <==
\section{Prior rules for Termination} % Calling this related work might be effective. Should I present Katoen's new AST rule as well here?

We now discuss a few existing proof rules for probabilistic termination.
% These form the components of our rules.
In all rules in this work, we denote the $\CFG$ that these rules operate over by $\cG = (L, V, l_{init}, \bfx_{init}, \ordMapsTo, G, \sfPr, \sfUp)$ and the set of states of $\cG$ reachable from the initial state $(l_{init}, \bfx_{init})$ $\Sigma_\cG$.

\VRS{It's a bit hard for me to imagine how we could write this in the form of Natural Deduction / Hoare Logic. I'm leaving this like this for now.}
\begin{proofrule}[Variant Rule for $\AST$ \cite{McIverMorganBook}] % Can't add Lemma 7.5.1 here for some reason
    \label{proofrule:ast-variant}
    If there is a partial function $U : L \times \setOfIntegers^{|L|} \to \setOfIntegers$ defined over $\Sigma_\cG$ that yields
    (1) bounds $L$ and $H$ such that for all states $(l, \bfx) \in \Sigma_\cG$, $L \leq U(l, \bfx) < R$, and
    (2) an $\epsilon > 0$ such that, for each state $(l, \bfx) \in \Sigma_\cG$,
    \begin{enumerate}[label=(\alph*)]
        \item if $(l, \bfx)$ is a terminal state, $U(l, \bfx) = 0$.
        \item if $(l, \bfx)$ is a deterministic, assignment, or nondeterministic state, $U(l', \bfx') < U(l, \bfx)$ for every successor $(l', \bfx')$.
        \item if $(l, \bfx)$ is a probabilistic state, $\sum \sfPr(l, l')[\bfx] > \epsilon$ over all successor states $(l', \bfx')$ with $U(l', \bfx') < U(l, \bfx)$.
    \end{enumerate}
    Then, $\cG$ is $\AST$.
\end{proofrule}

The soundness and limited completeness of \cref{proofrule:ast-variant} was proved by \citet[Lemma 7.6.1]{McIverMorganBook}.
\begin{lemma}
    \label{lem:completeness-mciver-morgan-rule}
    \cref{proofrule:ast-variant} is sound for all $\AST$ programs, and complete for finite state $\AST$ $\CFG$s.
\end{lemma}

We now introduce the notion of the \emph{stochastic invariants} \cite{ChatterjeeNZ17}
and \emph{stochastic invariant indicators} \cite{ChatterjeeGMZ22} % Not sure if we should remove this now.
to discuss the next rule.

   \begin{definition}[Stochastic Invariants]
    \label{def:stochastic-invariants}
    Let $\cG$ be a $\CFG$ $(L, V, l_{init}, \allowbreak \bfx_{init}, \ordMapsTo, G, \sfPr, \sfUp)$, $f$ be a scheduler of $\cG$, and $(runs_\cG, \cF_\cG, p_f)$ be the probability space representing the semantics of $\cG$ under $f$. 
    Suppose $SI$ is a subset of states $(l, \bfx)$ reachable from $(l_{init}, \bfx_{init})$, and $p$ is a probability value. 
    The tuple $(SI, p)$ is a \emph{stochastic invariant} (SI) if, under any scheduler $f$, the probability mass of the collection of runs beginning from $(l_{init}, \bfx_{init})$ leaving $SI$ is bounded above by $p$, i.e., 
    $$
    \sup p_f\left[ \rho \in runs_\cG \mid \exists n \in \setOfNaturals \cdot \rho[n] \not\in SI  \right] \leq p % Putting and _f under sup makes it look bad idk 
    $$
\end{definition}



Stochastic Invariants are equivalently characterized as Stochastic Invariant Indicators \cite{ChatterjeeGMZ22}. 
\begin{definition}[Stochastic Invariant Indicator]
    Let $\cG$ be the $\CFG$ $(L, V, l_{init}, \allowbreak \bfx_{init}, \ordMapsTo, G, \sfPr, \sfUp)$. 
    A tuple $(u_{SI}, p)$ is a stochastic invariant indicator (SI-indicator) if $p$ is a probability value and $u_{SI} : L \times \setOfIntegers^{|L|} \to \setOfReals$ is a partial function such that $u_{SI}(l_{init}, \bfx_{init}) \leq p$, and for all states $(l, \bfx)$ reachable from $(l_{init}, \bfx_{init})$, 
    \begin{enumerate}
        \item $u_{SI}(l, \bfx) \geq 0$. 
        \item if $(l, \bfx)$ is a deterministic, assignment, or nondeterministic state, then $u_{SI}(l, \bfx) \geq u_{SI}(l', \bfx')$ for every successor $(l', \bfx')$. 
        \item if $(l, \bfx)$ is a probabilistic state, then $u_{SI}(l, \bfx) \geq \sum \sfPr((l, l'))[\bfx] \times u_{SI}(l', \bfx')$ over all possible successor states $(l', \bfx')$. 
    \end{enumerate}
  \end{definition}
  
These properties ensure that SI-indicators begin with a value that's at most $p$, remain non-negative, and in expectation, don't increase over the course of an execution.
\citet{ChatterjeeGMZ22} proved that every Stochastic Invariant can be transformed into a SI-Indicator, and used these indicators in combination with a simple $\AST$ rule to claim a sound and complete proof technique to prove lower bounds on the probability of termination.


A final proof rule for Lower Bounds, introduced by \citet{FengCSKKZ23}, involves constraining the execution space by strengthening the guards over every transition.
This transformed program is typically finite-state, and therefore easier to analyze.

\begin{proofrule}[Guard Strengthening rule \cite{FengCSKKZ23}]
    \label{proofrule:katoen-guard-rule}
    Let $\varphi$ be a \emph{guard augmentation predicate}: a boolean expression over $V \cup L$ that is true at $(l_{init}, \bfx_{init})$.

    Denote by $\cG_\varphi$ the $\CFG$ $(L, V, l_{init}, \allowbreak \bfx_{init}, \ordMapsTo_\varphi, G_\varphi, \sfPr_\varphi, \sfUp_\varphi)$ obtained in the following way:
    \begin{enumerate}
        \item Set $G_\varphi(\tau) \coloneqq G(\tau) \land \varphi$ for each $\tau \in \ordMapsTo$.
        \item Set $\ordMapsTo \coloneqq \ordMapsTo \cup \{(l, l) \mid l \in L\}$.
        \item Now, set $G_\varphi(l, l) = \lnot \varphi$ for all self loops $(l, l) \in \ordMapsTo_\varphi$.
        \item For probabilistic locations $l$, set $\sfPr_\varphi(l, l) \coloneqq 1$.
        \item For assignment locations $l$, set $\sfUp_\varphi(l, l) = (1, x_1)$. % Necessary because of the $\CFG$ syntax. Note that certain deterministic locations become nondeterministic now, but I'm not sure if it's best to comment on that.
    \end{enumerate}
    Then, $\termProb(\cG) \geq \termProb(\cG_\varphi)$.
\end{proofrule}

The soundness of \cref{proofrule:katoen-guard-rule} has been proved for programs without nondeterminism \cite{FengCSKKZ23}.
% It can be extended to programs with nondeterminism quite easily.
It can be shown to be complete for programs where the variables are known to only range over the integers. % Not sure if I should talk about this now.
It highly applicable, going so far to be useful toward proving lower bounds on the famously unintuitive 3-D random walker.
Applications of \cref{proofrule:katoen-guard-rule} typically craft the guard augmentation predicate $\varphi$ to yield a finite state $\cG_\varphi$.
